CogWAM: Aligning Semantic Cognition with World Action Modeling via Event-Driven Interfaces

Robot policies increasingly incorporate semantic reasoning and future-world prediction, yet combining these capabilities does not guarantee that local predictions and actions remain aligned with task progress. We introduce CogWAM, a cognition-guided world-action model that establishes an explicit semantic interface between task reasoning and world-action learning through a persistent Semantic State, which stores completed task events and the active subtask. CogWAM updates this state only when observations indicate semantic transitions, allowing task-level context to persist across multiple action chunks. To bridge semantic context with physical prediction and control, CogWAM employs progress-conditioned WORLD and ACTION queries that selectively extract task-relevant information for future-world prediction and action generation. During training, the Semantic State provides shared task-progress context for both branches, while inference removes the future-prediction branch and directly generates actions from observations and the maintained state. We further introduce semantic training strategies to improve transition learning and closed-loop conditioning. Without additional robot-action pretraining, CogWAM achieves 15.56 / 11.70 % Score/SR on RoboDojo and state-of-the-art performance on BiCoord, while real-world experiments demonstrate closed-loop dual-arm manipulation with 16.4 fewer Semantic State regenerations than step-wise updating.

==> algo/algo_label.tex <==
\begin{algorithm}[t]
\caption{Offline construction of semantic supervision}
\label{alg:semantic_annotation}
\begin{algorithmic}[1]
\Require Recorded episode $\mathcal{R}$ of length $T$,
         task instruction $\ell$, and task metadata $\mu$
\Ensure Dense semantic targets
        $\mathcal{Y}
        =\{(d_t^\star,\Delta m_t^\star,s_t^\star)\}_{t=1}^{T}$

\State $\mathcal{C}=(c_1,\ldots,c_K)
       \gets \Call{ResolveChecklist}{\mathcal{R},\mu}$
\Comment{ordered task stages}

\State $(\mathcal{F},\mathcal{J})
       \gets \Call{SampleFrames}{\mathcal{R},\mu}$
\Comment{sampled frames and original indices}

\State $\boldsymbol{b}
       \gets \Call{VLM-BoundaryAnnotation}
       {\mathcal{F},\mathcal{J},\ell,\mathcal{C},T}$
\Comment{stage completion boundaries}

\State $\boldsymbol{b}
       \gets \Call{ParseAndValidate}{\boldsymbol{b},K,T}$

\State $\mathcal{P}
       \gets \Call{BoundariesToSpans}
       {\mathcal{C},\boldsymbol{b},T}$

\For{$t=1,\ldots,T$}
    \State $s_t^\star
           \gets \Call{ActiveStage}{\mathcal{P},t}$

    \If{$\Call{IsTransition}{\mathcal{P},t}$}
        \State $d_t^\star\gets\texttt{UPDATE}$
        \State $\Delta m_t^\star
               \gets\Call{CompletedStage}{\mathcal{P},t}$
    \Else
        \State $d_t^\star\gets\texttt{KEEP}$
        \State $\Delta m_t^\star\gets\varnothing$
    \EndIf
\EndFor

\State \Return
$\mathcal{Y}
=\{(d_t^\star,\Delta m_t^\star,s_t^\star)\}_{t=1}^{T}$
\end{algorithmic}
\end{algorithm}
